Teacher Guided Training: An Efficient Framework for Knowledge Transfer

The remarkable performance gains realized by large pretrained models, e.g., GPT-3, hinge on the massive amounts of data they are exposed to during training. Analogously, distilling such large models to compact models for efficient deployment also necessitates a large amount of (labeled or unlabeled) training data. In this paper, we propose the teacher-guided training (TGT) framework for training a high-quality compact model that leverages the knowledge acquired by pretrained generative models, while obviating the need to go through a large volume of data. TGT exploits the fact that the teacher has acquired a good representation of the underlying data domain, which typically corresponds to a much lower dimensional manifold than the input space. Furthermore, we can use the teacher to explore input space more efficiently through sampling or gradient-based methods; thus, making TGT especially attractive for limited data or long-tail settings. We formally capture this benefit of proposed data-domain exploration in our generalization bounds. We find that TGT can improve accuracy on several image classification benchmarks as well as a range of text classification and retrieval tasks.

==> 030_prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

\section{Background and notation}


Recall that we assume that the label set $\YCal$ with $K$ classes takes the form $[K]:= \{1,\ldots, K\}$. We use $\FC$ to denote the collection of potential classification models that the learning methods is allowed to select from, namely {\em function class} or {\em hypothesis set}:
\begin{align}
\FC \subseteq \{ \XCal \to \real^K\},
\end{align}
which is a subset of all functions that map elements of the instance space $\XCal$ to the elements of $\real^K$. 

Given a classification loss function $\ell : \real^{K} \times \YCal \to \real$ and a model $f : \XCal \to \real^K$ and a sample $\SCal^{\rm labled}_n = \{(x_i, y_i)\}_{i \in [n]}$ generated from $\DCal$, we define the {\em empirical risk} for $f \in \FC$ as follows.
\begin{align}
\label{eq:er-f-l}
R_{\ell, f}(\SCal^{\rm labled}_n) := \frac{1}{n}\sum\nolimits_{i \in [n]}\ell\big(f(x_i), y_i\big).
\end{align}
Further, we define the {\em population} risk for $f \in \FC$ associated with data distribution $\DCal$ as follows.
\begin{align}
\label{eq:pr-f-l}
R_{\ell, f}(\DCal) = \mathbb{E}_{X,Y \sim \DCal}[\ell(f(X), Y)].
\end{align}
Note that, when the loss function $\ell$ is clear from the context, we drop $\ell$ from the notation and simply use $R_{f}(\SCal^{\rm labled}_n)$ and  $R_{f}(\DCal)$ to denote the the empirical and populations risks for $f$, respectively.

Let $\SCal_n = \{x_i\}_{i \in [n]}$ be a set of $n$ {\em unlabeled} samples generated from $\DCal_{X}$. Then, given a teacher model $h : \XCal \to \real^K$ and a distillation loss $\ell_{\drm}: \real^K \times \real^K \to \real^K \to \real$, we define the {\em empirical (distillation) risk} for $f \in \FC$ to be
\begin{align}
\label{eq:distill-er}
    R^{h}_{\ell_{\drm}, f}(\SCal_n) := \frac{1}{n}\sum_{i \in [n]} \ell_{\drm}\big(f(x_i), h(x_i)\big).
\end{align}
Accordingly, the {\em population (distillation) risk} for $f \in \FC$ is defined as
\begin{align}
\label{eq:distill-pr}
R^{h}_{\ell_{\drm}, f}(\DCal) := \mathbb{E}_{X \sim \DCal_X}\left[\ell_{\drm}(f(X), h(X))\right].
\end{align}
Again, when $\ell_{\drm}$ is clear from the context, we simply use $R^{h}_{f}(\SCal_n)$ and $R^{h}_{f}(\DCal)$ to denote the empirical and population distillation risk for $f$, respectively. 

Note that, for a (student) function class $\FC$ and a teacher model $h$, $\ell_d$ produces an induced function class $\GC_{\ell_{\drm}, h}(\FC)$, defined as 
\begin{align}
\label{eq:distill-induced-fc}
\GC^{h}_{\ell_{\drm}, \FC} := \{x \mapsto  \ell_{\drm}(f(x), h(x)) : f \in \FC\}.
\end{align}

\begin{definition}[Rademacher complexity of $\GC^{h}_{\ell_{\drm}, \FC}$]
Given a sample $\SCal_n = \{x_i\}_{i \in [n]} \sim \DCal_{X}^n$ and a vector $\bm{\sigma} = (\sigma_i,\ldots, \sigma_m) \in \{+1, -1\}$ with $n$ i.i.d. Bernoulli random variable, empirical Rademacher complexity $\RF_{\SCal_n}\big(\GC^{h}_{\ell_{\drm}, \FC}\big)$ and Rademacher complexity $\RF_n\big(\GC^{h}_{\ell_{\drm}, \FC}\big)$ are defined as 
\begin{align}
\label{eq:distill-empirical-rc}
\RF_{\SCal_n}(\GC^{h}_{\ell_{\drm}, \FC}) = \frac{1}{n}\mathbb{E}_{\bm{\sigma}}\Big[ \sup_{g \in \GC^{h}_{\ell_{\drm}, \FC}} \sum_{i=1}^{n}\sigma_i g(x_i)\Big],
\end{align}
and
\begin{align}
\label{eq:distill-rc}
\RF_{n}(\GC^{h}_{\ell_{\drm}, \FC}) = \mathbb{E}_{\SCal \sim \DCal_{X}^n}\left[ \RF_{\SCal_n}(\GC^{h}_{\ell_{\drm}, \FC})\right].
\end{align}
\end{definition}
---------------------------------------{\color{red} STOP HERE} ----------------- Still working below


\section{Preliminaries}
\label{app:prelim}
\todoasr{This subsubsection will eventually be moved to Section 3 and/or appendix.}
For a loss function $\ell$ and a function class $\FC$, let us define an induced function class
\begin{align}
\label{eq:extened-fc}
\GC_{\ell} = \big\{ (x, y) \mapsto \ell(f(x), y) : f \in \FC\big\}.
\end{align}
Now, given a sample $\SCal = \{(x_i, y_i)\}_{i \in [n]} \sim \DCal^n$ and a vector $\bm{\sigma} = (\sigma_i,\ldots, \sigma_m) \in \{+1, -1\}$ with $n$ i.i.d. Bernoulli random variable, empirical Rademacher complexity $\RF_{\SCal}(\GC_{\ell})$ and Rademacher complexity $\RF_n(\GC_{\ell})$ are defined as 
\begin{align}
\RF_{\SCal}(\GC_{\ell}) = \frac{1}{n}\mathbb{E}_{\bm{\sigma}}\left[ \sup_{g \in \GC_{\ell}} \sum_{i=1}^{n}\sigma_i g(x_i, y_i)\right]
\end{align}
and
\begin{align}
\RF_{n}(\GC_{\ell}) = \mathbb{E}_{\SCal \sim \DCal^n}\left[ \RF_{\SCal}(\GC_{\ell})\right] %
\end{align}


\subsection{Multiclass classification}

In this paper, we focus on a multiclass classification task where given an instance $x \in \XCal$ the objective is to predict its true label $y \in \YCal$. Let $\DCal := \DCal_{X, Y}$ denote the underlying (joint) data distribution over the instance and label spaces for the task. Moreover, we use $\DCal_{X}$ and $\DCal_{Y | X = x}$ to denote the marginal distribution over the instance space $\XCal$ and the conditional label distribution for a given instance $x$, respectively. 

In a supervised setting, one assumes access to $n$ i.i.d. labeled samples $\SCal := \{(x_i, y_i)\}_{i \in [n]}$, generated from $\DCal$. Given $\SCal$, the objective is to learn a scorer function $f: \XCal \to \real^{|\YCal|}$ that assigns a relevance score $f_y(x)$ to label $y$ for an input instance $x$. For a fixed scorer function $f$, its final prediction on $x \in \XCal$ is defined by 
\begin{align}
\hat{y}_{f, x} = \arg\max_{y \in \YCal} f_y(x).
\end{align}
Accordingly, the misclassification error or {\em risk} of $f$ takes the form:
\begin{align}
&{\rm R}_{f}(\DCal) = \mathbb{P}_{X,Y}\{\hat{Y}_{f, X} \neq Y\} = \mathbb{E}_{X,Y \sim \DCal}[\mathds{1}_{\{\hat{Y}_{f, X} \neq Y\}}] \nonumber \\
&\qquad \quad= \mathbb{E}_{X,Y \sim \DCal}[\ell_{0/1}(f(X), Y)],
\end{align}
where $\mathds{1}_{\{ \cdot \}}$ and $\ell_{0/1}:\real^{|\YCal|} \times \YCal \to \{0, 1\}$ denote the indicator function and $0/1$ loss functions, respectively.
Assuming that $\FC$ denote the function class consisting of all score functions of interest, one can learn the scorer function by minimizing an empirical estimate of the misclassification error based on the available labeled set $\SCal$:
\begin{align}
\label{eq:emp-err}
{\rm R}_{f}(\SCal) := { \frac{1}{n} \sum\nolimits_{i \in [n]}\ell_{0/1}(f(X), Y)}.  
\end{align}
Since it's computationally intractable to minimize the $\ell_{0/1}$-based objective in \cref{eq:emp-err}, one typically employs a surrogate of $\ell_{0/1}$, say $\ell:\real^{|\YCal|} \times \YCal \to \real$, and solves the following {\em empirical risk minimization} problem.
\begin{align}
\label{eq:erm-obj}
\widehat{f}_n  = \arg\min_{f \in \FC} { \frac{1}{n} \sum\nolimits_{i \in [n]}\ell(f(X), Y)} {~:={\rm R}_{f, \ell}(\SCal)},    
\end{align}
where ${\rm R}_{f,\ell}(\SCal)$ denote the {\em empirical} risk based on $\ell$. Note that, $${\rm R}_{f,\ell_{0/1}}(\SCal) = {\rm R}_{f,\ell}(\SCal).$$ Similarly, one can define the {\em population} risk based on $\ell$ as 
\begin{align}
{\rm R}_{f, \ell}(\DCal) = \mathbb{E}_{X,Y \sim \DCal}[\ell(f(X), Y)],
\end{align}
which reduces to ${\rm R}_{f}(\DCal)$ when $\ell = \ell_{0/1}$.

ERM and its variants have been extensively studied in the literature. Specifically, a large body of work focuses on analyzing the quality of the modeled produced by ERM~\citep{devroye2013probabilistic, mohri2018foundations}. Rademacher complexity based generalization bounds are among the most popular tools to relate the performance of the ERM solution with that of the best model in the function class $\FC$. In their most common form, these bounds state the following
\begin{align}
R_{\hat{f}_n, \ell}(\DCal) - R_{f^{\ast}, \ell}(\DCal)  &\leq 2\RC_n (\GC) + \OC\left(\frac{2\log 1/\delta}{n}\right),
\end{align}
where, for distribution $\DCal$, $\RC_n (\GC)$ denotes the Rademacher complexity of the function class
\begin{align}
\GC = \{ (x, y) \mapsto \ell \circ f : f \in \FC\}
\end{align}
and $f^{ast}$ denote the model with the lowest population risk in $\FC$, i.e., 
\begin{align}
f^{\ast} = \argmin_{f \in \FC} R_{f, \ell}(\DCal).
\end{align}
\todoasr{Define rademacher?}

Another class of generalization bounds that are sometimes more suitable for ananlysis rely on the variance of ERM objective associated with an individual function in  $\FC$. For $\epsilon > 0$ and $S_n = (x_1,\ldots, x_n)$, let $\NC(\epsilon, \FC(S_n), \|\cdot\|_{\infty})$ denote the covering number of the set $$\GC\{S_n\}:= \{(g(x_1),\ldots, g(x_n)) : g \in \GC\}.$$ Assuming that
$$ 
\MC(n) = \NC_{\infty}({1}/{n}, \GC, 2n) = \sup_{S \subset \XCal^n} \NC(\epsilon, \GC(S), \|\cdot\|_{\infty})
$$
and $\ell$ is a bounded loss function. Then, one can state the following generalization bounds hold for with probability at least $1-\delta$~\citep{Maurer2009_colt}:
\begin{align}
\label{eq:var-based-bound}
R_{f, \ell}(\DCal) &\leq  R_{f, \ell}(\SCal_n)  + \OC\Big(\sqrt{\frac{{\rm Var}(f)\cdot\log(\MC(n)/\delta)}{n}}  + \nonumber \\
&\qquad \frac{\log(\MC(n)/\delta)}{n}\Big) 
\end{align}



\subsection{Knowledge distillation}
Knowledge distillation or distillation~\citep{bucilua2006_compression, hinton2015_distilling} is a popular technique for model training that goes beyond simply relying on the labels provided with training samples. In its simplest form, distillation leverages the scores of one model, referred to as the teacher model, to provide supervision for the training of another model, namely the student model. In particular, let $h: \XCal \to \real^{K}$ be the scorer function of the teacher model. Then, given a labeled set $\SCal_n$, one typically solves the following optimization problem to train the student model via distillation.
\begin{align}
\label{eq:distill-obj}
\arg\min_{f \in \FC} \frac{1}{n}\sum_{i \in [n]}\ell(f(x), y) + \lambda \cdot \frac{1}{n}\sum_{i \in [n]} d(f(x), h(x)),
\end{align}
where $\lambda > 0$ and $d: \real^{K} \times \real^{K} \to \real$ denote the distance between the scores on $x$ provided by $f$ and $h$. A common choice for $d$ is the cross-entropy between the distributions defined by $f(x)$ and $h(x)$. Formally, for a score function $f$, let $p^f(x) \in \Delta_{[K]}$ be the probability distribution defined as follow.
\begin{align}
p^{f}_{y}(x) = {e^{\tau f_y(x)}}/{\sum_{y' \in [K]}e^{\tau f_{y'}(x)}},~~\forall~y \in [K].
\end{align}
Now, $d(f(x), h(x))$ can be defined using the standard cross-entropy function as
\begin{align}
\label{eq:dist-ce}
d(f(x), h(x)) = - \sum_{y \in [K]} p^{h}_{y}(x) \cdot \log p^{f}_{y}(x).
\end{align}
\begin{remark}
Note that the distance in \cref{eq:dist-ce} reduces to the standard softmax-based cross entropy loss when $p^h(x)$ is one-hot distribution defined by the true label $y$, 
\begin{align}
p^h_{y'}(x)  = \begin{cases}
1 & y' = y, \\
0 & \text{otherwise}.
\end{cases}
\end{align}
In this case, we have $d(f(x), h(x)) = - \log p^{f}_{y}(x)$, which is indeed the softmax-based cross entropy loss.
\end{remark}

Given a function class $\FC$ and a distance $d:\real^{K} \times \real^{K} \to \real$, one can define a distance over $\FC$ as follows:
\begin{align}
d(f, f'; \DCal_{X}) = \mathbb{E}_{\DCal_X} \left[d(f(X), f'(X))\right]~~\forall~f, f' \in \FC.
\end{align}
Thus, the distillation objective in \cref{eq:distill-obj} can be views as 
\begin{align}
\label{eq:distill-obj-i}
\arg\min_{f \in \FC} R_{f, \ell}(\SCal) + \lambda \cdot d(f, h; \SCal),
\end{align}
where $ d(f, h; \SCal)$ denotes an empirical estimate of $d(f, f'; \DCal_{X})$ based on the samples in $\SCal$. Alternatively, distillation process can be viewed as {\em restricted} empirical risk minimization, where function class $\FC$ is restricted based on the teacher model $h$:
\begin{align}
\label{eq:distill-obj-ii}
\argmin_{f \in \FC_{\gamma}(h, \SCal)} R_{f, \ell}(\SCal),
\end{align}
where $\gamma > 0$ depends on $\lambda$ and 
\begin{align}
\label{eq:FC-gamma}
 \FC_{\gamma}(h, \SCal) = \{f \in \FC~:~ d(f, h; \SCal) \leq \gamma\}.
\end{align}

\begin{remark}
\label{rem:self-distill}
{\em Self-distillation} is an special instantiation of distillation technique where student and teacher models have an identical architecture~\citep{furlanello18_self}. 
\end{remark}

\citet{foster2019selection} employ a notion of {\em data-dependent} hypothesis set to obtain the generalization bounds for the constrained ERM in \cref{eq:distill-obj-ii}. In particular, under the assumption that teacher $h$ is learned by an algorithm that is $\beta$-stable \cneeded, their generalization bound ensure that, for any $f \in \FC_{\gamma}{h, \SCal}$, 
\begin{align}
 &R_{f, \ell}(\DCal) \leq R_{f, \ell}(\SCal) + 2 \RF^{\diamond}_{m}(\GCal_{h}) + \nonumber \\ 
 &\qquad \qquad \qquad (1 + 2\mu\beta m)\sqrt{\frac{1}{2m}\log\left( \frac{1}{\delta}\right)}   
\end{align}

For the distillation objective that does not leverage one-hot labels, i.e.,
\begin{align}
\label{eq:distill-obj-unlabled}
\arg\min_{f \in \FC} d(f, h; \SCal),
\end{align}
\citet{menon21a} obtain the following version of the variance-based generalization bound in \cref{eq:var-based-bound}:
\begin{align}
&R_{f, \ell}(\DCal) \leq  R_{f, \ell}(\SCal_n)  + \OC\Big(\sqrt{\frac{{\rm Var}(f)\cdot\log(\MC(n)/\delta)}{n}}  + \nonumber \\
&\qquad \frac{\log(\MC(n)/\delta)}{n}\Big) + \OC\big(\mathbb{E}_{\DCal_X}\|h(X) - \DCal_{Y|X}\|_2\big),
\end{align}
where $\DCal_{Y|X}$ is treated as a vector in $\R^{K}$, $k$-th coordinate denoting the probability $\mathbb{P}(Y=k|X)$ under the data distribution $\DCal$.

\subsection{Semi-supervised learning via distillation}
Semi-supervised learning generalizes the supervised learning setting where the learner is provided with $m$ unlabeled instances $\UCal_m = \{x_i\}_{i \in [m]} \subset \XCal$ in addition to the $n$ labeled examples in $\SCal$. As discussed in Section~\ref{sec:related}, there a multiple recently proposed techniques for training in a semi-supervised setting that rely on generating pseudo labels for the unlabeled (and labeled) data. For example, the consistency regularization-based approaches~\citep{zhu2021rich, berthelot2019_mixmatch, sohn2020_fixmatch} employ the following strategy or a variant thereof, potentially after performing further augmentation on $\SCal_n$ and $\UCal_m$:
\begin{enumerate}
    \item First train a model based on the labeled data $f^{(1} \in \FC$, e.g., via ERM in \cref{eq:erm-obj}.
    \item Generate $\{f_l(x)\}_{x \in \SCal_n \cup \UCal_m}$ as pseudo-labels for both labeled and unlabeled sets. Subsequently, for $\lambda_{ss} > 0$ learn the final model via
    \begin{align}
    \label{eq:ss-self-obj}
       \argmin_{f \in \FC} R_{f, \ell}  + \lambda_{ss} \cdot d(f, f^{(1)}; \SCal_n \cup \UCal_m).
    \end{align}
\end{enumerate}
Note that the objective in \cref{eq:ss-distill-obj} is akin to performing self-distillation (cf.~\cref{eq:distill-obj-i} and  Remark~\ref{rem:self-distill}). Interestingly, the two-stage process highlighted above can be employed in multiple alternate iteration between steps 1 and 2. Interestingly, it is not necessary to restrict onself to utilizing the model under training to generate the pseudo labels. In particular, one can leverage a pretrained model $h$ for this purpose, which translates to employing distillation with the following objective.
\begin{align}
\label{eq:ss-distill-obj}
\argmin_{f \in \FC} R_{f, \ell}  + \lambda_{ss} \cdot d(f, h; \SCal_n \cup \UCal_m),
\end{align}
which, as illustrated in \cref{eq:distill-obj-ii}, is equivalent to the following {\em restricted} ERM:
\begin{align}
\label{eq:distill-obj-ii}
\argmin_{f \in \FC_{\gamma_{ss}}(h, \SCal_n \cup \UCal_m)} R_{f, \ell}(\SCal),
\end{align}
with $\gamma_{ss} > 0$ and $\FC_{\gamma_{ss}}(h, \SCal_n \cup \UCal_m)$ follows the notation introduced in \cref{eq:FC-gamma}. %


